Non Commutative Convolutional Signal Models in Neural Networks: Stability to Small Deformations

In this paper we discuss the results recently published in~[1] about algebraic signal models (ASMs) based on non commutative algebras and their use in convolutional neural networks. Relying on the general tools from algebraic signal processing (ASP), we study the filtering and stability properties of non commutative convolutional filters. We show how non commutative filters can be stable to small perturbations on the space of operators. We also show that although the spectral components of the Fourier representation in a non commutative signal model are associated to spaces of dimension larger than one, there is a trade-off between stability and selectivity similar to that observed for commutative models. Our results have direct implications for group neural networks, multigraph neural networks and quaternion neural networks, among other non commutative architectures. We conclude by corroborating these results through numerical experiments.

==> figures/50_asp.tex <==
%!TEX root = ../compiler_paper.tex


\def \scale { 1.2}
\def \unit  { \scale cm}




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%



% %% ----- Viridis color palette -----
% \definecolor{my_cp_col1}{RGB}{253, 231, 37}
% \definecolor{my_cp_col2}{RGB}{180, 222,44}
% \definecolor{my_cp_col3}{RGB}{94, 201, 98}
% \definecolor{my_cp_col4}{RGB}{33, 145, 140}
% \definecolor{my_cp_col5}{RGB}{59, 82, 139}
% \definecolor{my_cp_col6}{RGB}{68, 1, 84}

%----- Cividis color palette -----
\definecolor{my_cp_col1}{RGB}{0, 32, 81}
\definecolor{my_cp_col2}{RGB}{43, 68, 110}
\definecolor{my_cp_col3}{RGB}{105, 105, 112}
\definecolor{my_cp_col4}{RGB}{148, 143, 120}
\definecolor{my_cp_col5}{RGB}{202, 186, 106}
\definecolor{my_cp_col6}{RGB}{253, 234, 69}





%%%%%%%%%%%%%%%%%% Block styles %%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{set} = [ rectangle,
                    rounded corners = 0.4*\unit,
                    inner sep=0pt,
                    draw,
                    anchor = center ]


\tikzstyle{vector space} = [ set,
                             fill=my_cp_col1,
                             minimum width  = 3*\unit,
                             minimum height = 1.86*\unit]

\tikzstyle{endomorphisms} = [ vector space,
                              fill=my_cp_col3,
                              minimum height = 1.6*\unit]

\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_cp_col6,
                        minimum width = 1.5*\unit]


\tikzstyle{dot} = [circle,
                    minimum width  = 0.1*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{8}{8}\selectfont

\begin{tikzpicture}[-stealth, draw = black!99, scale = \scale]

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Vector space M
   \path (0,0) node [vector space] (M) {};
   \path (M.south) ++ (0, 0.2) node [above] {\textcolor{my_cp_col6}{$\ccalM$}};
   
   % Element of the vector space
   \path (M) ++ (0, +0.3) node [dot,color=my_cp_col6] (x) {};
   \path (x.south) node [below] {\textcolor{my_cp_col6}{$\bbx$}};             
   % Processing ---> rho(th)x
   \path (M) ++ (+1, +0.3) node [dot,color=my_cp_col6] (ex) {};
   \path (ex.south) node [below] {\textcolor{my_cp_col6}{$\rho(th)\bbx$}};
   
   % Processing ---> rho(ht)x
   \path (M) ++ (-1, +0.3) node [dot,color=my_cp_col6] (rex) {};
   \path (rex.south) node [below] {\textcolor{my_cp_col6}{$\rho(ht)\bbx$}}; 
     

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Space of endomorphisms
   \path (M.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End) {};
   \path (End.north) ++ (0.0, -0.2) node [below] {\textcolor{my_cp_col6}{$\text{End}(\ccalM)$}};   

   % Adding an endomorphism element 
   \path (End.center) ++ (0.5, -0.37) node [dot] (e) {};      
   \path (e) node [above right] {\textcolor{my_cp_col6}{$\rho(th)$}};  
   
   % Adding an endomorphism element 
   \path (End.center) ++ (-0.5, -0.37) node [dot] (re) {};      
   \path (re) node [above left] {\textcolor{my_cp_col6}{$\rho(ht)$}}; 
   
   % Arrow going from x to \rho(th)x
   \path (End.center) + (0.2,0.1) coordinate (c1);
   \path (End.center) + (0.8,0.1) coordinate (c2);   
   \path [draw, -stealth,color=my_cp_col5, thin] (x) .. controls (c1) and (c2) .. (ex);   

   % Arrow going from x to \rho(ht)x
   \path (End.center) + (-0.2,0.1) coordinate (c1);
   \path (End.center) + (-0.8,0.1) coordinate (c2);   
   \path [draw, -stealth,color=my_cp_col5, thin] (x) .. controls (c1) and (c2) .. (rex); 
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Algebra
   \path (End.north west) ++ (-0.5, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.2) node [below] {$\ccalA$};   
   
   % Adding an element of the algebra
   \path (A.center) ++ (+0.5,0) node [dot] (a) {};      
   \path (a) node [below left] {$th$};    
   
    % Adding an element of the algebra
   \path (A.center) ++ (-0.5,0) node [dot] (ra) {};      
   \path (ra) node [below ] {$ht$};

   % Arrow going from a to e = \rho(a)
   \path (End.west) + (-0.1,0.25) coordinate (c1);
   \path (End.east) + (+0.1,0.25) coordinate (c2);   
   \path [draw, -stealth, line width = 1.0, my_cp_col1] 
         (a) edge [bend left] node [above] {$\rho~~~$} (e);  
         
   % Arrow going from a to e = \rho(a)
   \path (End.west) + (-0.1,0.25) coordinate (c1);
   \path (End.east) + (+0.1,0.25) coordinate (c2);   
   \path [draw, -stealth, line width = 1.0, my_cp_col1] 
         (ra) edge [bend right] node [below] {$\rho~~~$} (re);        


\end{tikzpicture}

}








==> figures/fig_1_tikz_source.tex <==
% !TEX root = ../compiler_paper.tex




\def \scale { 1.5}
\def \unit  { \scale cm}




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

% %% ----- Viridis color palette -----
% \definecolor{my_cp_col1}{RGB}{253, 231, 37}
% \definecolor{my_cp_col2}{RGB}{180, 222,44}
% \definecolor{my_cp_col3}{RGB}{94, 201, 98}
% \definecolor{my_cp_col4}{RGB}{33, 145, 140}
% \definecolor{my_cp_col5}{RGB}{59, 82, 139}
% \definecolor{my_cp_col6}{RGB}{68, 1, 84}

%----- Cividis color palette -----
\definecolor{my_cp_col1}{RGB}{0, 32, 81}
\definecolor{my_cp_col2}{RGB}{43, 68, 110}
\definecolor{my_cp_col3}{RGB}{105, 105, 112}
\definecolor{my_cp_col4}{RGB}{148, 143, 120}
\definecolor{my_cp_col5}{RGB}{202, 186, 106}
\definecolor{my_cp_col6}{RGB}{253, 234, 69}



%%%%%%%%%%%%%%%%%% Block styles %%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{set} = [ rectangle,
rounded corners = 0.2*\unit,
inner sep=0pt,
draw,
anchor = center ]

\tikzstyle{vector space} = [ set,
fill=my_cp_col1,
minimum width  = 1*\unit,
minimum height = 1.25*\unit]

\tikzstyle{vectorspace2} = [ set,
fill=my_cp_col2,
minimum width  = 0.5*\unit,
minimum height = 1.25*\unit]

\tikzstyle{endomorphisms} = [ vector space,
fill=my_cp_col3,
minimum height = 1*\unit,
minimum width = 1*\unit]


\tikzstyle{endomorphisms2} = [vector space,
fill=my_cp_col3,
minimum height = 0.7*\unit,
minimum width = 0.7*\unit]


\tikzstyle{algebra} = [ endomorphisms,
fill=my_cp_col6,
minimum width = 1*\unit,
minimum height = 1*\unit]

\tikzstyle{dot} = [ circle,
minimum width  = 0.1*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = center ]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{8}{8}\selectfont
	
	\begin{tikzpicture}[-stealth, draw = black!99, scale = \scale]
	
	
	
	%%----------------------------------
	%%--------- Vector space M ------
	%%----------------------------------
	
	\path (0,0) node [vector space,opacity=1] (M) {};
	\path (M.south) ++ (0, 0.2) node [above] {\textcolor{my_cp_col6}{$\ccalM$}};
	


   %%-----------------------------------------
   %%----------- Sum of Vector spaces M ------
   %%-----------------------------------------    
   
   \path (M.south)+(2.5,-1) node [vectorspace2,opacity=1,anchor=south] (V1) {};
   \path (V1.east) ++ (0.3, 0) node []  {$\ccalU_1$};
   \path (V1.north) node [opacity=1,anchor=south] (bigsum1) {$\bigoplus$};
    
   \path (bigsum1.north)+(0,0) node [vectorspace2,opacity=1,anchor=south] (V2) {};
   \path (V2.east) ++ (0.3, 0) node []  {$\ccalU_2$};
   \path (V2.north) node [opacity=1,anchor=south] (bigsum2) {$\bigoplus$};
   
   \path (bigsum2.north)+(0,0) node [vectorspace2,opacity=1,anchor=south] (V3) {};
   \path (V3.east) ++ (0.3, 0) node []  {$\ccalU_3$};     

   % Box covering the whole sum
   \path (V1.south west) + (-0.1,-0.1) coordinate (caux);
   \draw[color=my_cp_col5,line width=0.1mm] (caux) rectangle +(0.7,4.7);



   %%--------------------------------------------------------------------------
   %%------------ Homomorphisms associated to Vector Spaces in the Sum --------
   %%--------------------------------------------------------------------------
   
   \path (V1.west) ++ (-0.5, 0) node [endomorphisms2] (EndV1) {\textcolor{my_cp_col6}{$\phi_1 (a)$}};
   \path (EndV1.north) ++ (0, 0) node [anchor=south]  {$\text{End}(\ccalU_1)$};
   
   \path (V2.west) ++ (-0.5, 0) node [endomorphisms2] (EndV2) {\textcolor{my_cp_col6}{$\phi_2 (a)$}};
   \path (EndV2.north) ++ (0, 0) node [anchor=south]  {$\text{End}(\ccalU_2)$};
   
   \path (V3.west) ++ (-0.5, 0) node [endomorphisms2] (EndV3) {\textcolor{my_cp_col6}{$\phi_3 (a)$}};
   \path (EndV3.north) ++ (0, 0) node [anchor=south]  {$\text{End}(\ccalU_3)$};


	
	
	
	%%-------------------------------------------
	%%--------- Space of endomorphisms -----
	%%-------------------------------------------
	
	\path (M.north) ++ (0, 0.3) 
	node [endomorphisms, anchor=south] (End) {};
	\path (End.north) ++ (0.0, 0) node [below] {\textcolor{my_cp_col6}{$\text{End}(\ccalM)$}};   
	
	% Adding the adjoint of the element
	\path (End.center) ++ (0,-0.2) node [dot] (e) {};      
	\path (e) node [right] {\textcolor{my_cp_col6}{$\rho(a)$}}; 
	
	
	
		

    %%--------- Symbol of Isomorphism -----------
    
    \path (M.north east) ++ (0.3, 0) node [anchor=south west]  {$\cong$};
	
	
	
	
	
	%%--------------------------------------
	%%--------------- Algebra --------------
	%%--------------------------------------
	
	\path (End.north west) ++ (-0.5, 0) 
	node [algebra, anchor = north east,opacity=1] (A) {};   
	\path (A.north) ++ (-0.1,-0.1) node [below] {$\ccalA$};   
    
	% Adding the adjoint of the element
	\path (A.center) ++ (0,-0.2) node [dot] (a) {};      
	\path (a) node [left] {$a$};   
	

	
	
%% -----------------------------------------------------
%%-------------------Drawing the arrows-----------------
%% -----------------------------------------------------

% Frequency 3
\draw [->,line width=0.5mm, opacity=0.8,color=my_cp_col1,dashed] (a)..controls (-1,3) and (1,3)..(EndV3.west) node[midway,above,rotate=0,color=my_cp_col1] {$\phi_{3}$};
	
% Frequency 2
\draw [->,line width=0.5mm, opacity=0.8,color=my_cp_col1,dashed] (a)..controls (-0.8,2.6) and (1,2.6)..(EndV2.west) node[midway,above,rotate=0,color=my_cp_col1] {$\phi_{2}$};	
	
% Frequency 1
\draw [->,line width=0.5mm, opacity=0.8,color=my_cp_col1,dashed] (a)..controls (-1.5,-1.5) and (1,-1.5)..(EndV1.west) node[midway,above,rotate=0,color=my_cp_col1] {$\phi_{1}$};	
	
	
%----- Homomorphism from A to EndM
%-- Arrow going from a to e = \rho(a)
   \path (End.west) + (-0.1,0.25) coordinate (c1);
   \path (End.east) + (+0.1,0.25) coordinate (c2);   
   \path [draw, -stealth, line width = 1.0, my_cp_col1] 
         (a) edge [bend left] node [above] {$\rho~~~$} (e);  


	
	
	\end{tikzpicture}
	
}








==> figures/gnn_block_diagram_single_feature_uncolored.tex <==
% !TEX root = ../00_gnn_eusipco.tex

%\definecolor{my_blue}{rgb}{0, 0, 0.4}
\definecolor{my_blue}{rgb}{0.0314, 0.3569, 1.0000}

\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 3.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=my_blue!50!cyan]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 3.0*\unit,
                             fill = gray!30!white]
                             %fill = mygreen!15]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.5)}
\def \deltaoutput    {( 0.0,-0.9)}
\def \deltalayer     {3.0}
\def \deltaconnector {0.95}
\def \deltasigma     {( 4, 0.0)}
\def \deltafeature   {1.5}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\mathbf{y}_{1}  = \rho_{1}(a)\mathbf{x}}$}
\def \two   {$\displaystyle{\mathbf{y}_2  =  \rho_{2}(a)\mathbf{x}_{1}}$}
\def \three {$\displaystyle{\mathbf{y}_3  = \rho_{3}(a)\mathbf{x}_{2}}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\displaystyle{\mathbf{z}_{1} = {\eta_{1}} \Big[\, \mathbf{y}_1 \, \Big]}$}
\def \sigmatwo   {$\displaystyle{\mathbf{z}_{2} = {\eta_{2}} \Big[\, \mathbf{y}_2 \, \Big]}$}
\def \sigmathree {$\displaystyle{\mathbf{z}_{3} = {\eta_{3}} \Big[\, \mathbf{y}_3 \, \Big]}$}
\def \proyone   {$\displaystyle{\mathbf{x}_{1} = {P_{1}} \Big[\, \mathbf{z}_1 \, \Big]}$}
\def \proytwo   {$\displaystyle{\mathbf{x}_{2} = {P_{2}} \Big[\, \mathbf{z}_2 \, \Big]}$}
\def \proythree   {$\displaystyle{\mathbf{x}_{3} = {P_{3}} \Big[\, \mathbf{z}_3 \, \Big]}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\mathbf{x}$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  \path (L1 F1) ++ \deltasigma node [nonlinearity] (L1 F2)      {\proyone};
  % Draw connectors for Layer 1
  %\path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{z}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{y}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 F1.east) -- node [above] {$\mathbf{z}_1$} (L1 F2.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  \path (L2 F1) ++ \deltasigma node [nonlinearity] (L2 F2)      {\proytwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\mathbf{y}_2$} (L2 F1.west);
  \path[draw, -stealth] (L2 F1.east) -- node [above] {$\mathbf{z}_2$} (L2 F2.west);  
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  \path (L3 F1) ++ \deltasigma node [nonlinearity] (L3 F2)      {\proythree};
  % Draw connectors for Layer 2
  %\path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\mathbf{z}_3$} (L3 F1.west);
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\mathbf{y}_3$} (L3 F1.west);
  \path[draw, -stealth] (L3 F1.east) -- node [above] {$\mathbf{z}_3$} (L3 F2.west); 

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.south) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F2.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F2.south) -- node [below right] {$\mathbf{x}_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\mathbf{x}_1$} (L2 Filter1.north);
  % From layer 2 to layer 3
  \path (L2 F2.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F2.south) -- node [below right] {$\mathbf{x}_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\mathbf{x}_2$} (L3 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L3 F2.south) -- ++ \deltaoutput -- ++ (0.3, 0) 
                        node [right]{$\mathbf{x}_3$};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg} 
      % Shading for Layer 1  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 %minimum width  = 10.75*\unit,
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 1};
       \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{1}\in\mathcal{M}_{2}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{1}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{1},\mathbf{z}_{1}\in\mathcal{M}_{1}$};
      % Shading for Layer 2  
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 2};
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{2}\in\mathcal{M}_{3}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{2}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{2},\mathbf{z}_{2}\in\mathcal{M}_{2}$};
      % Shading for Layer 3  
      \path (L1 Filter1.west |- L3 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{3}\in\mathcal{M}_{\text{out}}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{3}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{3},\mathbf{z}_{3}\in\mathcal{M}_{3}$};
  \end{pgfonlayer}

\end{tikzpicture}} 


==> v02/sec_SpectOP.tex <==
%!TEX root = journal_AlgNN_v08.tex

\section{Spectral Operators}\label{sec:spectopt}
Before we proof the theorems presented in previous section, it is important to discuss the concept of \textit{Fourier decomposition} in the context of representation theory of algebras. We want to highlight specially the role of the filters when a representation is compared to its perturbed version. In particular, we will show that there are essentially two factors that can cause  differences between operators and their perturbed versions, the eigenvalues\footnote{As we will show later, this is indeed a particular case of a general notion of homomorphism between the algebra and an irreducible subrepresentation of $\mathcal{A}$.} and eigenvectors. Additionally, we show how the algebra can only affect one of those sources. This is consistent with the fact that differences in the eigenvectors of the operators only affect the constants that are associated to the stability bounds.

We highlight that the concept of spectral decomposition exploited extensively in traditional signal processing can be considered as a particular case of the concept of direct sums\footnote{When considering representations of non-compact groups this concept is insufficient and it is replaced for the more general notion of \textit{direct integral of Hilbert spaces}~\cite{folland2016course,deitmar2014principles}} of \textit{irreducible} representations. In this section we provide some basic definitions from the representation theory of algebras and its connection with the notion of spectral decomposition of signals in algebraic neural networks.  This will be useful and necessary in Section~\ref{sec:proofofTheorems} as the norm of the operators considered can be calculated in the terms of an spectral representation. We start with the following definition.
%%
%%------------------------Subsection---------------------------------
%\subsection{Finite and Countable infinite Dimensional Representations}
\begin{definition}
Let $(\mathcal{M},\rho)$ be a representation of $\mathcal{A}$. Then, a representation $(\mathcal{U},\rho)$ of $\mathcal{A}$ is a \textbf{subrepresentation} of  $(\mathcal{M},\rho)$ if $\mathcal{U}\subseteq\mathcal{M}$ and $\mathcal{U}$ is invariant under all operators $\rho(a)~\forall~a\in\mathcal{A}$, i.e. $\rho(a)u\in\mathcal{U}$ for all $u\in\mathcal{U}$ and $a\in\mathcal{A}$. A representation $(\mathcal{M}\neq 0,\rho)$ is \textbf{irreducible} or simple if the only subrepresentations of $(\mathcal{M}\neq 0,\rho)$ are $(0,\rho)$ and $(\mathcal{M},\rho)$.
\end{definition}
%
The class of irreducible representations of an algebra $\mathcal{A}$ is denoted by $\text{Irr}\{\mathcal{A}\}$. Notice that the zero vector space and $\mathcal{M}$ induce themselves subrepresentations of $(\mathcal{M},\rho)$. In order to state a comparison between representations the concept of \textit{homomorphism between representations} is introduced in the following definition.
%%
%%------------------------ Definition -----------------------------------------
\begin{definition}\label{def:homrep}
Let $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ be two representations of an algebra $\mathcal{A}$. A homomorphism or \textbf{interwining operator} $\phi:\mathcal{M}_{1}\rightarrow\mathcal{M}_{2}$ is a linear operator which commutes with the action of $\mathcal{A}$, i.e.
\begin{equation}
\phi(\rho_{1}(a)v)=\rho_{2}(a)\phi(v).
\label{eq:interwinop}
\end{equation}
A homomorphism $\phi$ is said to be an isomorphism of representations if it is an isomorphism of vectors spaces. 
\end{definition}
%%
%%
Notice from definition~\ref{def:homrep}  a substantial difference between the concepts of isomorphism of vector spaces and  isomorphism of representations. In the first case we can consider that two arbitray vector spaces of the same dimension (finite) are isomorphic, while for representations that condition is required but still the condition in eqn.~(\ref{eq:interwinop}) must be satisfied. For instance, as pointed out in~\cite{repthysmbook} all the irreducible 1-dimensional representations of the polynomial algebra $\mathbb{C}[t]$ are non isomorphic.

As we have discussed before, the vector space $\mathcal{M}$ associated to $(\mathcal{M},\rho)$  provides the space where the signals are modeled. Therefore, it is of central interest to determine whether it is possible or not to \textit{decompose} $\mathcal{M}$ in terms of simpler or smaller spaces consistent with the action of $\rho$.  We remark that for any two representations $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ of an algebra $\mathcal{A}$, their direct sum is given by the representation $(\mathcal{M}_{1}\oplus\mathcal{M}_{2},\rho)$ where $\rho(a)(\mathbf{x}_{1}\oplus\mathbf{x}_{2})=(\rho_{1}(a)\mathbf{x}_{1}\oplus\rho_{2}(a)\mathbf{x}_{2})$. We introduce the concept of indecomposability in the following definition.
%%
%%------------------------ Definition ------------------------------------------
\begin{definition}\label{def:indecomprep}
A nonzero representation $(\mathcal{M},\rho)$ of an algebra $\mathcal{A}$ is said to be \textbf{indecomposable} if it is not isomorphic to a direct sum of two nonzero representations.
\end{definition}
%%
%%
Indecomposable representations provide the \textit{minimum units of information} that can be extracted from signals in a given space when the filters have a specific structure (defined by the algebra)~\cite{barot2014introduction}. The following theorem provides the basic building block for the decomposition of finite dimensional representations.
%%
%%-----------------------------Theorem-------------------------------------------
\begin{theorem}[Krull-Schmit, \cite{repthybigbook}]\label{theorem:krullschmitdecomp}
Any finite dimensional representation of an algebra can be decomposed into a finite direct sum of indecomposable subrepresentations and this decomposition is unique up to the order of the summands and up to isomorphism. 
\end{theorem}
%%
%%
The uniqueness in this result means that if $(\oplus_{r=1}^{r}V_{i},\rho)\cong(\oplus_{j=1}^{s}W_{j},\gamma)$ for indecomposable representations $(V_{j},\rho_{j}),(W_{j},\gamma_{j})$, then $r=s$ and there is a permutation $\pi$ of the indices such that $(V_{i},\rho_{i})\cong (W_{\pi(j)},\gamma_{\pi(j)})$~\cite{repthybigbook}. Although theorem~\ref{theorem:krullschmitdecomp} provides the guarantees for the decomposition of representation in terms of indecomposable representations, it is not applicable when infinite dimensional representations are considered. However, it is possible to overcome this obstacle taking into account that irreducible representations are indecomposable~\cite{repthysmbook,repthybigbook}, and they can be used then to build representations that are indecomposable. In particular, \textit{irreducibility} plays a central role to decompose the invariance properties of the images of $\rho$ on $\text{End}(\mathcal{M})$~\cite{repthybigbook}. Representations that allow a decomposition in terms of subrepresentations that are irreducible are called \textit{completely reducible} and its formal description is presented in the following definition.
%%
%%-----------------------------Definition-----------------------------------------
\begin{definition}[~\cite{repthybigbook}]\label{def:complredu}
 A representation $(\mathcal{M},\rho)$ of the algebra $\mathcal{A}$ is said to be \textbf{completely reducible} if $(\mathcal{M},\rho)=\bigoplus_{i\in I}(\mathcal{U}_{i},\rho_{i})$ with irreducible subrepresentations $(\mathcal{U}_{i},\rho_{i})$. The \textbf{length} of $(\mathcal{M},\rho)$ is given by $\vert I\vert$.
\end{definition}
%%
%%
%Irreducible representations are indecomposable, therefore by using irreducible representations it is possible to decompose an arbitrary representation where the minimum component in the decomposition has an \textit{invariance property}.  

For a given $(\mathcal{U},\rho_{\mathcal{U}})\in\text{Irr}\{\mathcal{A}\}$ the sum of all irreducible subrepresentations of $(V,\rho_{V})$ that are equivalent (isomorphic) to $(\mathcal{U},\rho_{\mathcal{U}})$ is represented by $V(\mathcal{U})$ and it is called the $\mathcal{U}$-homogeneous component of $(V,\rho_{V})$. This sum is a direct sum, therefore it has a length that is well defined and whose value is called the \textit{multiplicity} of $(\mathcal{U},\rho_{\mathcal{U}})$ and is represented by $m(\mathcal{U},V)$~\cite{repthybigbook}. Additionally, the sum of all irreducible subrepresentations of $(V,\rho_{V})$ will be denoted as $\text{soc}\{V\}$. It is possible to see that a given representation $(V,\rho_{V})$ is completely reducible if and only if $(V,\rho_{V})=\text{soc}\{S\}$~\cite{repthybigbook}. The connection between $\text{soc}\{V\}$ and $V(\mathcal{U})$ is given by the following proposition. 
%%
%%---------------------------Proposition-------------------------------------
\begin{proposition}[Proposition 1.31~\cite{repthybigbook}]\label{prop:repdirectsum1}
Let $(V,\rho_{V})\in\mathsf{Rep}\{A\}$. Then $\text{soc}\{V\}=\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}V(S)$.
\end{proposition}
%%
%%
Now, taking into account that any homogeneous component $V(\mathcal{U})$ is itself a direct sum we have that 
\begin{equation}
\text{soc}\{V\}\cong\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}S^{\oplus m(\mathcal{U},V)}.
\label{eq:repdirectsumtot}
\end{equation}
Equation~(\ref{eq:repdirectsumtot}) provides the building block for the definition of Fourier decompositions in algebraic signal processing~\cite{algSP1}. With all these concepts at hand we are ready to introduce the following definition.
%%
%%-----------------------------Definition------------------------------------------
\begin{definition}[Fourier Decomposition]\label{def:foudecomp}
For an algebraic signal model $(\mathcal{A},\mathcal{M},\rho)$ we say that there is a spectral or Fourier decomposition of $(\mathcal{M},\rho)$ if
\begin{equation}
(\mathcal{M},\rho)\cong\bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})}
 \label{eq:foudecomp1}
\end{equation}
where the $(\mathcal{U}_{i},\phi_{i})$ are irreducible subrepresentations of $(\mathcal{M},\rho)$. Any signal $\mathbf{x}\in\mathcal{M}$ can be therefore represented by the map $\Delta$ given by 
\begin{equation}
\begin{matrix} 
\Delta: & \mathcal{M} \to \bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})} \\ & \mathbf{x}\mapsto \hat{\mathbf{x}}
 \end{matrix}
 \label{eq:foudecomp2}
\end{equation}
known as the Fourier decomposition of $\mathbf{x}$ and the projection of $\hat{\mathbf{x}}$ in each $\mathcal{U}_{i}$ are the Fourier components represented by $\hat{\mathbf{x}}(i)$.
\end{definition}
%%
%%
%\begin{figure}
% \centering\includegraphics[scale=1,angle=0]{../figures/fig9.pdf}
%  \caption{Diagram indicating the maps and the spaces when a completely reducible representation $(\mathcal{M},\rho)$ is decomposed as a direct sum of irreducible subrepresentations.}
%  \label{fig_3}
%\end{figure}
%%
%%
Notice that in eqn.~(\ref{eq:foudecomp1}) there are two sums, one dedicated to the non isomorphic subrepresentations (external) and another one (internal) dedicated to subrepresentations that are isomorphic. In this context, the sum for non isomorphic representations indicates the sum on the \textit{frequencies} of the representation while the sum for isomorphic representations a sum of components associated to a given frequency. It is also worth pointing out that $\Delta$ is an interwining operator, therefore, we have that $\Delta(\rho(a)\mathbf{x})=\rho(a)\Delta(\mathbf{x})$. As pointed out in~\cite{algSP0} this can be used to define a convolution operator as $\rho(a)\mathbf{x}=\Delta^{-1}(\rho(a)\Delta(\mathbf{x}))$. The projection of a filtered signal $\rho(a)\mathbf{x}$ on each $\mathcal{U}_{i}$ is given by $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and the collection of all this projections is known as the \textit{spectral representation} of the operator $\rho(a)$. Notice that $\phi_{i}(a)\hat{\mathbf{x}}(i)$ translates to different operations depending on the dimension of $\mathcal{U}_{i}$. For instance, if $\text{dim}(\mathcal{U}_{i})=1$, $\hat{\mathbf{x}}(i)$ and $\phi_{i}(a)$ are scalars while if $\text{dim}(\mathcal{U}_{i})>1$ and finite $\phi_{i}(a)\hat{\mathbf{x}}(i)$ is obtained as a matrix product.
%
%
%In many important applications the $\mathcal{U}_{i}$ in eqn.~(\ref{eq:foudecomp1}) are one dimensional spaces~\cite{algSP0,algSP1,algSP3}, that when seen as homogeneous components of a representation $(V,\rho_{V})$  became of particular interest as they are connected with the traditional concepts of eigenspaces and eigenvalues~\cite{repthybigbook}. Indeed, eigenspaces can be considered particular cases of the so called \textit{weight spaces}, introduced in the following definition.
%%%
%%%---------------------------Definition-----------------------------------------
%\begin{definition}[Weight spaces~\cite{repthybigbook}]\label{def:weightspaces}
%Let $(\mathcal{U},\phi)$ be a 1-dimensional representation of an algebra $\mathcal{A}$. Then the $\mathcal{U}-$homogeneous component $V(\mathcal{U})$ is given by
%\begin{equation}
%V(\mathcal{U})=\left\lbrace v\in V\vert \rho(a)v=\phi(a)v~\forall~a\in\mathcal{A}\right\rbrace 
%\label{eq:weightspaces}
%\end{equation}
%if $V(\mathcal{U})\neq 0$, then $\phi$ is called a \textbf{weight} of the representation $(V,\rho_{V})$ and $V(\mathcal{U})$ is called the corresponding \textbf{weight space}.
%\end{definition}
%%%
%%%
%In the context of definition~\ref{def:weightspaces} it is important to point out that when $\mathcal{A}=\mathbb{K}[t]$ and  $\phi(t)=\lambda\in\mathbb{K}$, $V(\mathcal{U})$ is the usual eigenspace for the eigenvalue $\lambda$ of the endomorphism $\rho(t)$. However when the algebra is not polynomial eqn.(~\ref{eq:weightspaces}) offers a generalization that allows to define more general spectral representations. 

%When considering definition~(\ref{def:foudecomp}) and eqn.(\ref{eq:foudecomp2}) with one dimensional subrepresentations the spectral representation of the operator $\rho(a)$ is given by
%\begin{equation}
%\rho(a)\mathbf{x}=\sum_{i}\hat{\mathbf{x}}(i)\phi_{i}(a)\mathbf{u}_{i}
%\label{eq:spectopt}
%\end{equation}
%where $\mathbf{u}_{i}$ is the basis vector associated to $\mathcal{U}_{i}$.
%%
%%-------------------------Remark--------------------------------------------------------------
\begin{remark}\label{remark:interpSpecFilt}\normalfont
The spectral representation of an operator indicated as $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and eqns.~(\ref{eq:foudecomp1}) and~(\ref{eq:foudecomp2}) highlight one important fact that is essential for the discussion of the results in Section~\ref{sec:proofofTheorems}. For a completely reducible representation $(\mathcal{M},\rho)\in\mathsf{Rep}\{\mathcal{A}\}$ the connection between the algebra $\mathcal{A}$ and the spectral representation is \textit{exclusively} given by $\phi_{i}(a)$ which is acting on $\hat{\mathbf{x}}(i)$, therefore, it is not possible by the selection of elements or subsets of the algebra to do any modification on the spaces $\mathcal{U}_{i}$ associated to the irreducible components in eqn.(\ref{eq:foudecomp1}). As a consequence, when measuring the similarities between two operators $\rho(a)$ and $\tilde{\rho}(a)$ associated to $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively, there will be two sources of error. One source of error that can be modified by the selection of $a\in\mathcal{A}$ and another one that will be associated with the differences between spaces $\mathcal{U}_{i}$ and $\tilde{\mathcal{U}}_{i}$, which are associated to the direct sum decomposition of $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively. This point was first elucidated in~\cite{fern2019stability} for the particular case of GNNs, but it is part of a much more general statement that becomes more clear in the language of algebraic signal processing. 
\end{remark}
%%
%%
%%------------------------------Subsection----------------------------
%%
%\subsection{Examples}
%%
%\subsubsection{CNNs}
\begin{example}[Discrete signal processing]\normalfont
In CNNs the filtering is defined by the polynomial algebra $\mathcal{A}=\mathbb{C}[t]/(t^{N}-1)$, therefore, in a given layer the spectral representation of the filters is given by
%
\begin{multline*}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\left(e^{-\frac{2\pi ij}{N}}\right)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i},
\end{multline*}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$ and where the $\mathbf{u}_{i}(v)=\frac{1}{\sqrt{N}}e^{\frac{2\pi jvi}{N}}$ are the column vectors of the traditional DFT matrix, while $\phi_{i}(t)=e^{-\frac{2\pi ji}{N}}$ is the eigenvalue associated to $\mathbf{u}_{i}$. Here $\hat{\mathbf{x}}$ represents the DFT of $\mathbf{x}$.
\end{example}
%%
%%---------------------------------Subsection-----------------------------------
\begin{example}[Graph signal processing]\normalfont
Taking into account that the filtering in each layer of a GNN is defined by a polynomial algebra, the spectral representation of the filter is given by
%
\begin{multline}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}=
\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\lambda_{i}^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
\label{eq:specopgnn}
\end{multline}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$, and where the $\mathbf{u}_{i}$ are given by the eigenvector decomposition of $\rho(t)=\mathbf{S}$, where $\mathbf{S}$ could be the adjacency matrix or the Laplacian of the graph, while $\phi_{i}(t)=\lambda_{i}$ being $\lambda_{i}$ the eigenvalue associated to $\mathbf{u}_{i}$. The projection of $\mathbf{x}$ in each subspace $\mathcal{U}_{i}$ is given by $\hat{\mathbf{x}}(i)=\langle\mathbf{u}_{i}, \mathbf{x}\rangle$, and if $\mathbf{U}$ is the matrix of eigenvectors of $\mathbf{S}$ we have the widely known representation $\hat{\mathbf{x}}=\mathbf{U}^{T}\mathbf{x}$~\cite{gamagnns}.
\end{example}
%%
%%-------------------Example--------------------------------
\begin{example}[Group signal processing]\label{example:specopGroupCNNs}
\normalfont
Considering the Fourier decomposition on  general groups~\cite{steinbergrepg,terrasFG,fulton1991representation}, we obtain the spectral representation of the algebraic filters as
\begin{equation*}
\boldsymbol{a}\ast\mathbf{x}=\sum_{u,h\in G}\boldsymbol{a}(uh^{-1})\sum_{i,j,k}\frac{d_{k}}{\vert G\vert}\hat{\mathbf{x}}\left(\boldsymbol{\varphi}^{(k)}\right)_{i,j}\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu,
\end{equation*}
where $\hat{\mathbf{x}}(\boldsymbol{\varphi}^{(k)})$ represents the Fourier components associated to the $k$th irreducible representation with dimension $d_{k}$ and $\boldsymbol{\varphi}^{(k)}$ is the associated unitary element. We can see that the $k$th element in this decomposition is $\sum_{i,j}\mathbf{x}(\varphi^{(k)})_{i,j}\sum_{u,h}\frac{d_{k}}{\vert G\vert}\boldsymbol{a}(uh^{-1})\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu$.
\end{example}
%%
%%-------------------Subsection--------------------------------
%\subsubsection{CNNs, with infinite dimensional representations}
\begin{example}[Graphon signal processing]\normalfont
According to the spectral theorem~\cite{conway1994course,aliprantis2002invitation}, it is possible to represent the action of a compact normal operator $S$ as $S\mathbf{x}=\sum_{i}\lambda_{i}\langle\boldsymbol{\varphi}_{i},\mathbf{x}\rangle\boldsymbol{\varphi}_{i}$ where $\lambda_{i}$ and $\boldsymbol{\varphi}_{i}$ are the eigenvalues and eigenvectors of $S$, respectively, and $\langle\cdot\rangle$ indicates an inner product. Then, the spectral representation of the filtering of a signal in the layer $\ell$ is given by
\begin{equation*}
\rho_{\ell}\left(p(t)\right)\mathbf{x}
=
\sum_{i}p(\lambda_{i})\langle\mathbf{x},\boldsymbol{\varphi}_{i}\rangle\boldsymbol{\varphi}_{i}=\sum_{i}\phi_{i}(p(t))\hat{\mathbf{x}}_{i}\boldsymbol{\varphi}_{i},
\end{equation*}
where $\phi_{i}(p(t))=p(\lambda_{i})$.
\end{example}










==> v02/sec_aggalgnn.tex <==
%!TEX root =../compiler_paper.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{figure}
% \centering\includegraphics[scale=0.8,angle=0]{../figures/fig7b.pdf}
% \caption{Schematic representation of the algebraic signal model}
% \label{fig_1}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Algebraic Signal Processings} \label{sec_alg_filters}%{Representation Theory of Algebras and Signal Models}


Algebraic signal processing (ASP) provides a framework for understanding and generalizing traditional signal processing exploiting the representation theory of algebras~\cite{algSP0, algSP1, algSP2, algSP3}. In ASP, a signal model is defined as the triple
%
\begin{equation}\label{eqn_ASP_signal_model}
   (\ccalA,\ccalM,\rho),
\end{equation}   
%
in which $\ccalA$ is an associative algebra with unity, $\ccalM$ is a vector space with inner product, and $\rho:\ccalA\rightarrow\text{End}(\ccalM)$ is a homomorphism between the algebra $\ccalA$ and the set of endomorphisms in the vector space $\ccalM$. The elements in \eqref{eqn_ASP_signal_model} are tied together by the notion of a representation which we formally define next. In this paper we further restrict attention to commutative algebras $\ccalA$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Representation] \label{def_representation} A representation of the associative algebra $\ccalA$ is a vector space $\ccalM$ equipped with a homomorphism $\rho:\ccalA\rightarrow\text{End}(\ccalM)$, i.e., a linear map preserving multiplication and unit. 
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
When denoting a representation of a given algebra we will use a pair consisting of the vector space and the homomorphism, for instance with the notation in definition~\ref{def_representation} the representation of the algebra $\mathcal{A}$ is denoted by $(\mathcal{M},\rho)$. The class of representations of  an algebra $\mathcal{A}$ is denoted as $\mathsf{Rep}\{\mathcal{A}\}$.

In an ASP model, signals  are elements of the vector space $\ccalM$, and filters are elements of the algebra $\ccalA$. Thus, the vector space $\ccalM$ deteremines the objects of interest and the algebra $\ccalA$ the rules of the operations that define a filter. The homomorphism $\rho$ translates the abstract operators $a\in\ccalA$ into concrete operators $\rho(a)$ that act on signals $\bbx$ to produce filter outputs 
%
\begin{equation}\label{eqn_ASP_filter_outputs}
   \bby = \rho(a) \bbx.
\end{equation}   
%
The algebraic filters in \eqref{eqn_ASP_filter_outputs} generalize the convolutional processing of time signals -- see Example \ref{ex_DTSP}. Our goal in this paper is to use them to generalize convolutional neural networks (Section \ref{sec_Algebraic_NNs}) and to study their fundamental stability properties (Section \ref{sec:perturbandstability}). Generators, which we formally define next, are important for the latter goal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Generators] \label{def_generators} For an associative algebra with unity $\ccalA$ we say the set $\ccalG\subseteq\ccalA$ generates $\ccalA$ if all $a\in\ccalA$ can be represented as polynomial functions of the elements of $\ccalG$. We say elements $g\in\ccalG$ are generators of $\ccalA$ and we denote as $a=p_{\ccalA}(\ccalG)$ the polynomial that generates $a$.
\end{definition}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Definition \ref{def_generators} states that elements $a\in\ccalA$ can be built from the generating set as polynomials using the operations of the algebra. Given the role of representations in connecting the algebra $\ccalA$ with the signals $\bbx$ as per Definition \ref{def_representation} the representation $\rho(g)$ of a generator $g\in\ccalG$ will be of interest. In the context of ASP, these representations are called shift operators as we formally define next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Shift Operators]\label{def_shift_operators} 
Let $(\ccalM,\rho)$ be a representation of the algebra $\ccalA$. Then, if $\ccalG\subset\ccalA$ is a generator set of $\ccalA$, the operators $\bbS = \rho(g)$ with $g\in\ccalG$ are called shift operators. The set of all shift operators is denoted by $\ccalS$
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Given that elements $a$ of the algebra are generated from elements $g$ of the generating set, it follows that filters $\rho(a)$ are generated from the set of shift operators $\bbS=\rho(g)$. In fact, if we have that $a=p_{\ccalA}(\ccalG)$ is the polynomial that generates $a$, the filter $\rho(a)$ is generated by 
%
\begin{equation}\label{eqn_filter_representation}
   \rho(a) = p_\ccalM \big(\rho(\ccalG)\big) 
           = p_\ccalM\big(\ccalS\big)
           = p\big(\ccalS\big),
\end{equation}
%
where the subindex $\ccalM$ signifies that the operations in \eqref{eqn_filter_representation} are those of the vector space $\ccalM$ -- in contrast to the polynomial $a=p_{\ccalA}(\ccalG)$ whose operations are those of the algebra $\ccalA$. In the last equality we drop the subindex $\ccalM$ to simplify notation as it is generally understood from context.

To clarify ideas it is instructive to consider some examples.

%%----------Polynomial and operators notation ---------
%\red{%
%\begin{equation}\label{eqn_DTSP_filter_outputs}
%   a =  p_{\ccalA}(\ccalG) = \sum_{k=0}^{K-1} h_k g^k 
%\end{equation}   
%
%\begin{equation}\label{eqn_DTSP_filter_outputs}
%   \rho(a) =  p_{\ccalM}(\ccalS) = \sum_{k=0}^{K-1} h_k \ccalS^k 
%\end{equation}   
%
%\begin{equation}\label{eqn_DTSP_filter_outputs}
%   \rho'(a) =  p_{\ccalR}(\lam) = \sum_{k=0}^{K-1} h_k \lam^k 
%\end{equation}   
%
%
%
%%
%}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{dtsp}
\setcounter{dtsp}{\theexample} 
\setcounter{example}{\thedtsp} 

\begin{example}[Discrete Time Signal Processing]\label{ex_DTSP}\normalfont Let $\ccalM = \ell^2$ be the space of square summable sequences $\bbx = \{x_n\}_{n\in\mbZ}$ and $\ccalA$ the algebra of polynomials with elements $a = \sum_{k=0}^{K-1} h_k t^k$. We consider the shift operator $S$ such that $S\bbx$ is the sequence with entries $(S\bbx)_n = x_{n-1}$. With the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k S^k$ the filters in \eqref{eqn_ASP_filter_outputs} are of the form 
%
\begin{equation}\label{eqn_DTSP_filter_outputs}
   \bby  \,=\, \rho\left(\sum_{k=0}^{K-1} h_k t^k\right) \bbx
         \,=\, \left(\sum_{k=0}^{K-1} h_k S^k\right) \bbx
         \,=\, \sum_{k=0}^{K-1} h_k S^k \bbx.
\end{equation}   
%
This is a representation of time convolutional filters \cite{algSP0}. Observe that the algebra of polynomials is generated by $g=t$ and that since $\rho(t) = S$ the shift operator $S$ generates the set of convolutional filters as it follows from \eqref{eqn_DTSP_filter_outputs}.\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{gsp}
\setcounter{gsp}{\theexample} 
\setcounter{example}{\thegsp} 

\begin{example}[Graph Signal Processing]\label{ex_GSP}\normalfont We retain the algebra of polynomials as in Example \ref{ex_DTSP} but we change the space of signals to the set of complex vectors with $N$ entries, $\ccalM =\mbC^N$. We interpret components $x_n$ of $\bbx\in\ccalM = \mbC^N$ as being associated with nodes of a graph with matrix representation $\bbS\in\mbC^{N\times N}$. With the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k \bbS^k$ the filters in~\eqref{eqn_ASP_filter_outputs} are of the form
%
\begin{equation}\label{eqn_GSP_filter_outputs}
   \bby \,=\, \rho\left(\sum_{k=0}^{K-1} h_k t^k\right) \bbx
        \,=\, \left(\sum_{k=0}^{K-1} h_k \bbS^k\right) \bbx
        \,=\, \sum_{k=0}^{K-1} h_k \bbS^k \bbx.
\end{equation}
%
This is a representation of the graph convolutional filters used in graph signal processing (GSP)~\cite{gsp_graphfilters,ortega_gsp}. Observe that \eqref{eqn_GSP_filter_outputs} and \eqref{eqn_DTSP_filter_outputs} are similar but represent different operations. In \eqref{eqn_GSP_filter_outputs} $\bbx$ is a vector and $\bbS^k$ a matrix power. In \eqref{eqn_DTSP_filter_outputs} $\bbx$ is a sequence and $S^k$ is the composition of the shift operator $S$. Their similarity arises from their common use of the algebra of polynomials. Their differences are because they use different vector spaces $\ccalM$ and different homomorphism functions $\rho$. \end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{dsp}
\setcounter{dsp}{\theexample} 
\setcounter{example}{\thedsp} 
%
\begin{example}[Discrete Signal Processing]\label{ex_DSP}\normalfont Make $\ccalM=\mbC^N$ and $\ccalA$ the algebra of polynomials in the variable $t$ and modulo $t^{N}-1$. Elements of $\ccalA$ are of the form $a = \sum_{k=0}^{K-1} h_k t^k$ but we must have $K\leq N$ and polynomial products use the rule $t^k = t^{k \mod N}$. Define the cyclic shift operator $C$ as one whose application to $\bbx\in\ccalM=\mbC^N$ yields a vector with components 
$(C \bbx)_n = x_{(n-1)\mod N}$. With the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k C^k$ the filters in~\eqref{eqn_ASP_filter_outputs} are of the form 
%
\begin{equation}\label{eqn_DSP_filter_outputs}
   \bby \,=\, \rho\left(\sum_{k=0}^{K-1} h_k t^k\right) \bbx
        \,=\, \left(\sum_{k=0}^{K-1} h_k C^k\right) \bbx
        \,=\, \sum_{k=0}^{K-1} h_k C^k \bbx.
\end{equation}
%
This is the representation of (cyclic) convolutional filters in discrete signal processing~\cite{algSP0}. We emphasize that the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k C^k$ is indeed a homomorphism because the cyclic shift operator $C$ satisfies $C^k = C^{k \mod N}$. \end{example}
%
%\begin{example}[Discrete Signal Processing]\label{ex_DSP}\normalfont Make $\ccalM=\mbC^N$ and $\ccalA$ the algebra of polynomials modulo $N$. Elements of $\ccalA$ are of the form $a = \sum_{k=0}^{K-1} h_k t^k$ but we must have $K<N$ and polynomial products use the rule $t^k = t^{k \mod N}$. Define the cyclic shift operator $C$ as one whose application to $\bbx\in\ccalM=\mbC^N$ yields a vector with components 
%$(C \bbx)_n = x_{(n-1)\mod N}$. With the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k C^k$ the filters in~\eqref{eqn_ASP_filter_outputs} are of the form 
%%
%\begin{equation}\label{eqn_DSP_filter_outputs}
%   \bby \,=\, \rho\left(\sum_{k=0}^{K-1} h_k t^k\right) \bbx
%        \,=\, \left(\sum_{k=0}^{K-1} h_k C^k\right) \bbx
%        \,=\, \sum_{k=0}^{K-1} h_k C^k \bbx.
%\end{equation}
%%
%This is the representation of (cyclic) convolutional filters in discrete signal processing~\cite{algSP0}. We emphasize that the homomorphism $\rho(a) = \sum_{k=0}^{K-1} h_k C^k$ is indeed a homomorphism because the cyclic shift operator $C$ satisfies $C^k = C^{k \mod N}$. \end{example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As is clear from Examples \ref{ex_DTSP}-\ref{ex_DSP}, the effect of the operator $\rho(a)$ on a given signal $\bbx$ is determined by two factors: The filter $a\in\ccalA$ and the homomorphism $\rho$. The filter $a\in\ccalA$ indicates the \textit{laws and rules} to be used to manipulate the signal $\bbx$ and $\rho$ provides a \textit{physical realization} of the filter $a$ on the space $\ccalM$ to which $\bbx$ belongs. For instance, in these three examples the filter $a=1 + 2t$ indicates that the signal is to be added to a transformed version of the signal scaled by coefficient $2$. The homomorphism $\rho$ in Example \ref{ex_DTSP} dictates that the physical implementation of this transformation is a time shift. The homomorphism $\rho$ in Example \ref{ex_GSP} defines a transformation as a multiplication by $\bbS$ and in Example \ref{ex_DSP} the homomorphism entails a cyclic shift. We remark that in order to specify the physical effect of a filter it is always sufficient to specify the physical effect of the generators. In all three examples, the generator of the algebra is $g=t$. The respective effects of an arbitrary filter $a$ are determined once we specify that $\rho(t) = S$ in Example \ref{ex_DTSP}, $\rho(t) = \bbS$ in Example \ref{ex_GSP}, or $\rho(t) = C$ in Example \ref{ex_DSP}. 

The flexibility in the choice of algebra and homomorphism allows for a very rich variety of signal processing frameworks. We highlight this richness with three more examples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{groupsp}
\setcounter{groupsp}{\theexample} 
\setcounter{example}{\thegroupsp} 

\begin{example}[Signal Processing on Groups]\normalfont \label{ex_groupsp} Let $\ccalM=\{\bbx: G\rightarrow\mathbb{C} \}=\{ \sum_{g\in G}\bbx(g)g\}$ be the set of functions defined on the group $G$ with values in $\mathbb{C}$ and $\ccalA=\ccalM$ the \textit{group algebra} with elements $\sum_{g\in G}\bba(g)g$. With a homomorphism given by $\rho(\bba)=\bba$ the filtering in~\eqref{eqn_ASP_filter_outputs} takes the form
\begin{equation}\label{eqn_group_filters}
\rho\left(\sum_{g\in G}\bba(g)g\right)\bbx=\sum_{g\in G}\bba(g)g\bbx=\sum_{g\in G}\sum_{h\in G}\bba(g)\bbx(h)gh,
\end{equation}
and making $u=gh$ we have
%
\begin{equation}\label{eqn_group_convolution}
   \sum_{g,h\in G} \bba(g)\bbx(h)gh 
             =\sum_{u,h\in G}\bba(uh^{-1})\bbx(h)u=\bba\ast\bbx .
\end{equation}
%
This is the standard representation of convolution of signals on groups~\cite{steinbergrepg,terrasFG,fulton1991representation}. We point out that \eqref{eqn_group_filters} and \eqref{eqn_group_convolution} hold for any group but that not all group algebras are commutative. Results in Section \ref{sec:stabilitytheorems} apply only when the group group algebra is commutative.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{wsp}
\setcounter{wsp}{\theexample} 
\setcounter{example}{\thewsp} 

\begin{example}[Graphon Signal Processing ]\normalfont \label{ex_wsp} Let $\ccalM=L^2([0,1])$ be the space of signals and $\ccalA$ the algebra of polynomials with elements $a = \sum_{k=0}^{K-1} h_k t^k$ with a homomorphism given by
$\rho(a)=\sum_{k=0}^{K-1} h_k S^k$ where
%
\begin{equation}\label{eqn_graphon_shift}
   \left(S\bbx\right)(u)=\int_{0}^{1}W(u,v)\bbx(v)dv,   
\end{equation}
%
where $W(u,v):[0,1]^{2}\rightarrow [0,1]$ is a graphon, i.e. bounded symmetric measurable function~\cite{lovaz2012large,segarragraphon}. Then, the filtering in~\eqref{eqn_ASP_filter_outputs} is of the form~\eqref{eqn_DTSP_filter_outputs}. 
%\begin{equation}\label{eqn_WSP_filter_outputs}
%   \bby = \left(\sum_{k=0}^{K-1} h_k \ccalS^k\right) \bbx
%        = \sum_{k=0}^{K-1} h_k \ccalS^k \bbx.
%\end{equation}
%
This is a representation of convolutional filters in the context of graphon signal processing~\cite{ruiz2020graphon}. \end{example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{example}[Lie Algebra Signal Processing ]\normalfont
%Let $\ccalM=\mathbb{R}^{N}$ be the space of signals and 
%\begin{equation}
%\ccalA=\frac{\mathbb{C}\langle x,y,z\rangle}{(xy-yx-2y,xz-zx-2z,yz-zy-x)}
%\end{equation}
%be the \textit{universal enveloping algebra}\footnote{The symbol $\mathbb{C}\langle x,y,z\rangle$ is the free algebra, i.e. the set of all words obtained by sequences of the symbols $x,y,z$ and their sums} of the Lie algebra $\mathfrak{sl}_{2}\mathbb{C}=\{A\in M_{2,2}(\mathbb{C})\vert \text{Tr}(A)=0\}$ with Lie bracket $[A,B]=AB-BA$. The elements in $\ccalA$ can be written as $a=\sum_{m,i,j,k}\alpha_{m,i,j,k}\boldsymbol{\pi}(x^{i},y^{j},z^{k})$ where $\alpha_{m,i,j,k}\in\mathbb{C}$ and $\boldsymbol{\pi}(x^{i},y^{j},z^{k})$ represents a permutation of the terms in $x^{i}y^{j}z^{k}$. The homomorphism $\rho$ is defined according to $\rho(x)=X$, $\rho(y)=Y$, $\rho(z)=Z$ where $X,Y,Z\in M_{N,N}(\mathbb{C})$, $XY-YX=2Y$, $XZ-ZX=2Z$ and $YZ-ZY=X$. As indicated in~\cite{hall_liealg,erdmann2006introduction} these sets of equations lead to a unique solution. Then, the filtering in~\eqref{eqn_ASP_filter_outputs} is of the form
%%
%\begin{multline}\label{eqn_liesp_filter_outputs}
%\rho\left(\sum_{m,i,j,k}\alpha_{m,i,j,k}\boldsymbol{\pi}\left(x^{i},y^{j},z^{k}\right)\right)\bbx\\
%=\sum_{m,i,j,k}\alpha_{m,i,j,k}\boldsymbol{\pi}\left(X^{i},Y^{j},Z^{k}\right)\bbx .
%\end{multline}   
%%
%These filters define convolutional signal processing in Lie Algebras.
%\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The choice of $\ccalA$ and $\rho$ provides means to leverage our knowledge of the signal's domain in its processing. The convolutional filters in \eqref{eqn_DTSP_filter_outputs} leverage the shift invariance of time signals and the filters in \eqref{eqn_DSP_filter_outputs} the cyclic invariance of periodic signals. The group convolutional filters in \eqref{eqn_group_convolution} generalize shift invariance to invariance with respect to an arbitrary group action. The graph convolutional filters in \eqref{eqn_GSP_filter_outputs} engender signal processing that is independent of node labeling \cite{gamagnns} and the graphon filters in Example \ref{ex_wsp} a generalization of this notion to dense domains~\cite{ruiz2020graphon}. Leveraging this structure is instrumental in achieving scalable information processing. In the following section we explain how neural network architectures combine algebraic filters as defined in \eqref{eqn_ASP_filter_outputs} with pointwise nonlinearities to attain signal processing that inherits the invariance properties of the respective algebraic filters. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}
\centering\input{./figures/gnn_block_diagram_single_feature_uncolored_01.tex}
  \caption{Algebraic Neural Network $\Xi=\{(\ccalA_{\ell},\ccalM_{\ell},\rho_{\ell})\}_{\ell=1}^{3}$ with three layers indicating how the input signal $\mathbf{x}$ is processed by $\Xi$ and mapped into $\mathbf{x}_{3}$.}
  \label{fig_6}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Algebraic Neural Networks}\label{sec_Algebraic_NNs}
%
With the concept of algebraic filtering at hand we define an algebraic neural network (AlgNN) as a stacked layered structure (see Fig.~\ref{fig_6})
 in which each layer is composed by the triple $(\ccalA_{\ell},\ccalM_{\ell},\rho_{\ell})$, which is an algebraic signal model associated to each layer. Notice that $(\ccalM_{\ell},\rho_{\ell})$ is a representation of $\ccalA_{\ell}$. The mapping between layers is performed by the maps $\sigma_{\ell}:\mathcal{M}_{\ell}\rightarrow\mathcal{M}_{\ell+1}$ that perform those operations of point-wise nonlinearity and pooling. Then, the ouput from the layer $\ell$ in the AlgNN is given by
%
\begin{equation}\label{eq:xl}
\bbx_{\ell}=\sigma_{\ell}\left(\rho_{\ell}(a_{\ell})\bbx_{\ell-1}\right)
\end{equation}
where $a_{\ell}\in\ccalA_{\ell}$, which can be represented equivalently as
%From now on we represent the map in eqn.~(\ref{eq:xl}) by
%that shows how a signal entering in the $\ell$th layer is processed and then mapped to the layer $\ell+1$ is given by 
%
\begin{equation}\label{eq:interlayeropalgnn}
\mathbf{x}_{\ell}=\Phi (\mathbf{x}_{\ell-1},\mathcal{P}_{\ell-1},\mathcal{S}_{\ell-1}),
\end{equation}
%
where $\mathcal{P}_{\ell}\subset\mathcal{A}_{\ell}$ highlights the properties of the filters and $\mathcal{S}_{\ell}$ is the set of shifts associated to $(\mathcal{M}_{\ell},\rho_{\ell})$. Additionally, the term $\Phi\left(\mathbf{x},\{ \mathcal{P}_{\ell} \}_{1}^{L},\{ \mathcal{S}_{\ell}\}_{1}^{L}\right)$ represents the total map associated to an AlgNN acting on a signal $\mathbf{x}$.
%%
%%------------------------SUBSECTION------------------------------
\subsubsection{Convolutional Features}
The processing in each layer can be performed by means of several families of filters, which will lead to several \textit{features}. In particular the feature $f$ obtained in the layer $\ell$ is given by
\begin{equation}\label{eqn:alg_feat}
\bbx_{\ell}^{f}=\sigma_{\ell}\left(\sum_{g=1}^{F_{\ell}}\rho_{\ell}\left(a_{\ell}^{gf}\right)\bbx_{\ell-1}^{g}\right),
\end{equation}
where $a_{\ell}^{fg}$ is the filter in $\ccalA_{\ell}$ used to process the $g$-th feature $\bbx_{\ell-1}^{g}$ obtained from layer $\ell-1$ and $F_{\ell}$ is the number of features. 
%%
%%------------------------SUBSECTION------------------------------
\subsubsection{Pooling}
As stated in~\cite{deeplearning_book} the pooling operation in CNNs helps to keep representations approximately invariant to small translations of an input signal, and also helps to improve the computational efficiency. In this work this operation is attributed  to the operator $\sigma_{\ell}$. In particular, we consider $\sigma_{\ell}=P_{\ell}\circ\eta_{\ell}$ where $P_{\ell}$ is a pooling operator and $\eta_{\ell}$ is a pointwise nonlinearity. The only property assumed from $\sigma_{\ell}$ is to be Lipschitz and to have zero as a fixed point, i.e. $\sigma_{\ell}(0)=0$. It is important to point out that $P_{\ell}$ projects elements from a given vector space into another.
%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[Traditional CNNs]\normalfont 
Traditional CNNs rely on the use of typical signal processing models and can be considered a particular case of an AlgNN  where the algebraic signal model is the same as in example~\ref{ex_DSP}. Consequently, 
the $f$th feature in layer $\ell$ is given by
\begin{equation}
\bbx_{\ell}^{f}=\sigma_{\ell}\left(\sum_{g=1}^{F_{\ell}}\sum_{i=1}^{K}h_{i}^{gf}\bbS_{\ell}^{i}\bbx_{\ell-1}^{g}\right),
\label{eq:featureCNN}
\end{equation}
where $\rho_{\ell}(t)=\bbS_{\ell}$. In this case $P_{\ell}$ is a sampling operator while typically $\eta_{\ell}(u)=\max\{0,u\}$.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[Graphon Neural Networks]\normalfont
In graphon neural networks the algebraic signal model in each layer corresponds to the one discussed in example~\ref{ex_wsp}. Consequently, the $f$th feature in layer $\ell$ has the form given in eqn.~\eqref{eq:featureCNN} considering a shift $S$ given according to eqn.~(\ref{eqn_graphon_shift}). It is worth noticing that in this case the signals in the inner layers of the network are meant to be represented using a finite number of eigenvectors of the shift operator. Then, if we denote by $\boldsymbol{\varphi}_{i}^{(\ell)}$ the eigenvectors of the graphon $W_{\ell}(u,v)$ associated to the $\ell$th layer $P_{\ell}$ is given by
\begin{equation}
P_{\ell}:\text{span}\left\lbrace \boldsymbol{\varphi}_{i}^{(\ell)}\right\rbrace_{i\in I}\rightarrow\text{span}\left\lbrace\boldsymbol{\varphi}_{j}^{(\ell+1)}\right\rbrace_{j\in J},
\end{equation}
where $I$ and $J$ are finite subsets of $\mathbb{N}$. Then, the signals in each $\ccalM_{\ell}$ are always functions of a continuous independent variable but with \textit{lower degrees of freedom} as $\ell$ increases.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   E   X   A   M   P   L   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[Group Neural Networks]\normalfont
In group neural networks the algebraic model is the same as specified in example~\ref{ex_groupsp}. Therefore, the $f$th feature in layer $\ell$ is given by
\begin{equation}
\bbx_{\ell}^{f}=\sigma_{\ell}\left(\sum_{n=1}^{F_{\ell}}\sum_{u,h\in G_{\ell}}\bba^{nf}_{(\ell)}(uh^{-1})\bbx_{\ell-1}(h)u\right).
\label{eq:featureGroupNN}
\end{equation}
where $G_{\ell}$ is the group associated to the $\ell$th layer and $\bba^{nf}_{(\ell)}$ are the coefficients of the filter associated to the feature $f$ in layer $\ell$. In this case $P_{\ell}:L^{2}(G_{\ell})\rightarrow L^{2}(G_{\ell+1})$,  where $L^{2}(G)$ is the set of signals of finite energy defined on the group $G$. If the groups $G_{\ell}$ are finite $P_{\ell}$ can be conceived as a typical projection mapping between $\mathbb{R}^{\vert G_{\ell}\vert}\rightarrow\mathbb{R}^{\vert G_{\ell+1}\vert}$.
\end{example}




==> v02/sec_algNN.tex <==

%%---------------------------------------------------------------------
%%---------SECTION: ALGEBRAIC NEURAL NETWORKS -------------------------
%%---------------------------------------------------------------------



\section{Algebraic Neural Networks}
\subsection{Convolution Feaures}
\subsection{Pooling}

==> v02/sec_discussion.tex <==
%%--------------------------------------------------------------------
%%---------------- SECTION: DISCUSSION--------------------------------
%%--------------------------------------------------------------------
%
\section{Discussion}\label{sec:discussion}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{./source_figs/plots_stability/graph_dilation_unstable.tex}\medskip
    \input{./source_figs/plots_stability/graph_dilation_stable.tex}    
   \caption{Filter properties and stability for algebraic operators considering algebras with a single generator. (Top) We depict a Lipschitz filter where it is possible to see that an arbitrary degree of selectivity can be achieved in any part of the spectrum. (bottom) We depict a Lipschitz integral filter where we can see how the magnitude of the filters tends to a constant value as the size of $\vert\lambda_{i}\vert$ grows. As a consequence there is no discriminability in one portion of the spectrum.}
 \label{fig_graph_dilation}
\end{figure}
%
%\medskip \noindent {\bf Perturbation analysis and selectivity in spectrum} 
The mathematical form of the notion of stability introduced in definition~(\ref{def:stabilityoperators1}), eqn.~(\ref{eq:stabilityoperators1}) is uncannily similar to the expressions associated to the stability conditions stated in~\cite{mallat_ginvscatt,bruna_iscn} when the perturbation operator $\tau$  considered was affecting directly the domain of the signals.  This is consistent with the fact that  the size of the perturbation on the operators is the size of an induced diffeomorphism $\mathbf{T}$ acting on $\text{End}(\mathcal{M})$. Measuring the size of perturbations in this way, although less intuitive, provides an alternative way to handle and interpret perturbations on irregular domains. 

The nature and severity of the perturbations, imposes restrictions on the behavior of the filters needed to guarantee stability. The more complex and severe the perturbation is the more conditions  on the filters are necessary to guarantee stability. This in particular has implications regarding to the selectivity of the filters in some specific frequency bands. The trade-off between stability and selectivity in the filters of the AlgNN can be measured by the size of the upper bounds in Theorems~\ref{theorem:HvsFrechet} up to~\ref{theorem:stabilityAlgNN1}, in particular, the size of $L_{0}$ and $L_{1}$ associated to the boundedness of the derivatives of the elements in $\mathcal{A}_{L0}$ and $\mathcal{A}_{L1}$. The smaller the value of $L_{0}, L_{1}$ the more stable the operators but the less selectivity we have. In Fig.~(\ref{fig_graph_dilation}) the properties in frequency of Lipschtiz and Lipschitz integral filters are depicted, where it is possible to see how the selectivity on portions of the spectrum is affected by properties that at the same time provide stability conditions for the perturbation models considered. 

It is important to remark that the function $\sigma_{\ell}=P_{\ell}\circ\eta_{\ell}$ composed by the projection operator $P_{\ell}$ and the nonlinearity function $\eta_{\ell}$ relocates information from one layer to the other performing a mapping between different portions of the spectrum associated to each of the spaces $\mathcal{M}_{\ell}$.  As $\eta_{\ell}$ maps elements of $\mathcal{M}_{\ell}$ onto itself,  we can see in light of the decomposition of $\mathcal{M}_{\ell}$ in terms of irreducible representations that 
$\eta_{\ell}$ is nothing but a relocator of information from one portion of the spectrum to the other. Additionally, the simplicity of $\eta_{\ell}$ provides  a rich variety of choices that can be explored in future research. 

The notion of differentiability between metric spaces or Banach spaces can be considered also using the notion of \textit{G\^ateaux derivative} which is considered a \text{weak} notion of differentiability. Although Gateaux differentiability is in general different from Fr\'echet  differentiability, it is possible to show that when $\text{dim}\left(\text{End}(\mathcal{M})\right)<\infty$ both notions are equivalent for Lipschtiz functions, but substantial differences may exist if $\text{dim}\left(\text{End}(\mathcal{M})\right)=\infty$ even if the functions are Lipschitz~\cite{benyamini2000geometric,lindenstrauss2012frechet}. 








==> v02/sec_multiplegenresults.tex <==
\green{

\section{Multiple Generators}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% THEOREM %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem:uppboundDHmultg}
Let $\mathcal{A}$ be an algebra with $m$ generators $\{g_{i}\}_{i=1}^{m}$ and $g_{i}g_{j}=g_{j}g_{i}$ for all $i,j\in\{1,\ldots m\}$. Let $(\mathcal{M},\rho)$ be a finite or countable infinite dimensional representation of $\mathcal{A}$ and $(\mathcal{M},\tilde{\rho})$ a perturbed version of $(\mathcal{M},\rho)$ related by the perturbation model in eqn.~(\ref{eq:perturbmod1}).  Then, if $p_{\mathcal{A}}\in\mathcal{A}_{L_{0}}\cap\mathcal{A}_{L_{1}}$ it holds that
%
\begin{multline}
\left\Vert D_{p_{\mathcal{M}}\vert\mathbf{S}_{i}}(\mathbf{S})\bbT(\bbS_{i})\right\Vert\leq
\\
(1+\delta_{0})L_{0}\sup_{\bbS_{i}\in\mathcal{S}}\Vert\bbT(\bbS_{i})\Vert +\left(1+q\delta\right)E_{q}L_{1}\sup_{\bbS_{i}\in\mathcal{S}}\Vert D_{\bbT}(\bbS_{i})\Vert
\label{eq:DHTSmultg}
\end{multline}
 \end{theorem}





--- CALCULATING the Frechet Derivative-------
\begin{proof}
$p(\mathbf{S})=p(\mathbf{S}_{1},\mathbf{S}_{2},\ldots,\mathbf{S}_{m})$, then

\begin{multline}
p(\mathbf{S}+\boldsymbol{\xi})-p(\mathbf{S})
\\
=\sum_{k_{1},\ldots,k_{m}=0}^{\infty}h_{k_{1},\ldots k_{m}}(\mathbf{S}_{1}+\boldsymbol{\xi}_{1})^{k_{1}}(\mathbf{S}_{2}+\boldsymbol{\xi}_{2})^{k_{2}}\cdots (\mathbf{S}_{m}+\boldsymbol{\xi}_{m})^{k_{m}}
\\
-\sum_{k_{1},\ldots,k_{m}=0}^{\infty}h_{k_{1},\ldots k_{m}}\mathbf{S}_{1}^{k_{1}}\mathbf{S}_{2}^{k_{2}}\ldots\mathbf{S}_{m}^{k_{m}}
\\
=D_{p\vert\mathbf{S}_{1}}(\mathbf{S})+\ldots +D_{p\vert\mathbf{S}_{m}}(\mathbf{S})+N(\boldsymbol{\xi})
\end{multline}
%
%
\end{proof}
}

==> v02/sec_quivrep.tex <==
%!TEX root = quiverSP_v00.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Quiver Representations}
\label{sec:quivrep}



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% FIGURE  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}
%	\centering
%\includegraphics[width=0.2\textwidth]{../figs/fig1.pdf}
%\includegraphics[width=0.2\textwidth]{../figs/fig2.pdf}
%\caption{A quiver $Q$ (left) and one  particular representation (right) of $Q$. $\mathcal{V}_{i}$ is a vector space associated to the node $i$ of the quiver while $\phi_{i,j}$ is a linear map between the spaces $\mathcal{V}_{i}$ and $\mathcal{V}_{j}$.}
%\label{fig:quiver1}
%\end{figure}


Informally speaking a quiver is a directed graph where multiple edges and loops are allowed, but in order to facilitate the introduction of the concept of representation we require a more formal definition that we introduce next. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def:quiver}
A quiver $Q$ is a quadruple $Q=(Q_{0},Q_{1},h,t)$ wehre $Q_{0}$ is a finite set of vertices, $Q_{1}$ is a finite set of arrows, and $h$ and $t$ are functions $Q_{1}\rightarrow Q_{0}$. For an arrow $a\in Q_{1}$, h(a) and $t(a)$ are called the head and the tail of $a$.
\end{definition}



%%
%%---------------------------------------Example---------------------------------------------------------------------
%%
\begin{example}\label{example:1}\normalfont
Let us consider the quiver indicated in Fig.~\ref{fig:quiver1} composed by the nodes $Q_{0}=\{1,2,3,4,5\}$ and the arrows $Q_{1}=\{a_{1,2}, a_{2,3},a_{2,2},a_{3,4},a_{3,5},a_{4,4},a_{4,1},a_{5,1}\}$. In this case we have that the functions $h$ and $t$ are given by $h(a_{i,j})=j$ and $t(a_{i,j})=i$.
\end{example}

Notice that the quiver itself does not offer anything new that has not been considered in the GSP literature. No structure is provided or associated to the graph. However, the notion of representation of a quiver provides the basic and formal components that can be used to associate information to the quiver in different ways. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%----------------------------------- DEFINITION -----------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
A representation $\boldsymbol{\pi}$ of a quiver $Q=(Q_{0},Q_{1},h,t)$ consists of a collection of vector spaces $\mathcal{V}_{i}$ associated to the \textbf{nodes} $i$, i.e. $\boldsymbol{\pi}(i)=\mathcal{V}_{i}$ for $i\in Q_{0}$ and a set of linear maps $\phi_{i,j}$ associated to the arrows, $\phi_{i,j}=\boldsymbol{\pi}(a_{i,j})$. Additionally, a representation $\boldsymbol{\theta}$ is called a subrepresentation of a representation $\boldsymbol{\pi}$ if $\boldsymbol{\theta}(x)$ is a subspace $\boldsymbol{\pi}(x)$ for all $x\in Q_{0}$, and $\boldsymbol{\pi}(a):\boldsymbol{\pi}(t(a))\rightarrow\boldsymbol{\pi}(h(a))$ restricts to $\boldsymbol{\theta}(a):\boldsymbol{\theta}(t(a))\rightarrow\boldsymbol{\theta}(h(a))$ for all $a\in Q_{1}$.
\end{definition}
%
%%------------------------------ End of DEFINITION -----------------------------------------------------------------

To show the versatility of a quiver representation to endow a directed graph with structure we recall the example~\ref{example:1} to discuss representations of the quiver indicated in Fig.~\ref{fig:quiver1} in the following example.



%%
%%---------------------------------------Example---------------------------------------------------------------------
%%

\begin{example}\normalfont
Taking into account the quiver discussed in example~\ref{example:1}, we can have the following representation: The vector spaces associated to the nodes are $\mathcal{V}_{1}=\mathbb{R}^{2}$, $\mathcal{V}_{2}=\mathbb{R}^{2,2}$, $\mathcal{V}_{3}=\mathbb{R}^{5,5}$, $\mathcal{V}_{4}=\mathbb{R}^{3}$, $\mathcal{V}_{5}=\mathbb{R}$ while the linear maps are given by
%
%
\begin{equation*}
\phi_{1,2}(\mathbf{x})=\mathbf{1}_{1\times2}\otimes\mathbf{x},\quad\phi_{1,3}(\mathbf{x})=\mathbf{1}_{1\times 5}\otimes\mathbf{x},\quad\phi_{2,2}(\mathbf{x})=3\bbx
\end{equation*}
%
%
\begin{equation*}
\phi_{2,3}(\bbx)=
\begin{pmatrix} 
\mathbf{x}                     & \mathbf{0}_{2\times 3}\\
\mathbf{0}_{3\times 2} &  \mathbf{0}_{3\times 3}
\end{pmatrix}
,\quad
\phi_{3,4}(\bbx)=[\bbx]_{(1:3),(1:3)},
\end{equation*}
%
%
\begin{equation*}
\quad \phi_{4,4}(\bbx)=\bbI_{4\times 4}\bbx,\quad \phi_{4,1}(\bbx)=[\bbx(1)+\bbx(2),\bbx(2)+\bbx(3)]^{T}
\end{equation*}
%
%
\begin{equation*}
\phi_{3,5}(\bbx)=\mathbf{1}_{1\times 5}\bbx\mathbf{1}_{5\times 1},\quad\phi_{5,1}(\bbx)=[\bbx,\bbx]^{T}
\end{equation*}
%
%
where $\mathbb{R}^{k,k}$ indicates the set of matrices of size $k\times k$ with entries in $\mathbb{R}$, $\mathbb{R}^{k}$ is the $k-$dimensional Euclidean space, $\mathbf{1}_{r\times k}$ and $\mathbf{0}_{r\times k}$ are the all ones array and the all zeros array of dimensions $r\times k$ while $\times$ denotes the Kronecker product. The symbol $[\bbx]_{(1:r),(1:k)}$ represents the array obtained keeping the first $r$ rows and the first $k$ columns of $\bbx$. 
\end{example}

%%
%%---------------------------------------End of Example---------------------------------------------------------------------
%%


%%
%%---------------------------------------Example---------------------------------------------------------------------
%%

\begin{example}\normalfont
\blue{Dear Hans: Here we can add an example of a quiver that arises naturally from an example in computational topology or anything related}
\end{example}

%%----------------------------------End of Example----------------------------------------------------------------


The notion of quiver representations  is naturally embeded in the context of the representation theory of algebras~\cite{repthysmbook,derksen2017introduction,kirillov2016quiver}. Therefore, it is possible to talk about irreducible representations, indecomposable representations and so on. In what follows we proceed to introduce these notions for quivers, which will be later used to define a signal processing framework. 

We start with a notion that will allow us to compare representations of a quiver.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
Let $\boldsymbol{\pi}_{1}$ and $\boldsymbol{\pi}_{2}$ be two representations of a quiver $Q=(Q_{0},Q_{1},h,t)$. We get a morphism $\phi:\boldsymbol{\pi}_{1}\rightarrow\boldsymbol{\pi}_{2}$ if we attach to every vertex $x\in Q_{0}$ a $\mathbb{C}-$linear map $\phi(x):\boldsymbol{\pi}_{1}(x)\rightarrow\boldsymbol{\pi}_{2}(x)$ such that for every $a\in Q_{1}$ the following diagram commutes
%
\begin{center}
\begin{tikzcd}
\boldsymbol{\pi}_{1}(t(a)) \arrow[r, "\boldsymbol{\pi}_{1}(a)"] \arrow[d, "\phi(t(a))"]
& \boldsymbol{\pi}_{1}(h(a)) \arrow[d, "\phi(h(a))" ] \\
\boldsymbol{\pi}_{2}(t(a)) \arrow[r, "\boldsymbol{\pi}_{2}(a)" ]
& \boldsymbol{\pi}_{2}(h(a)) 
\end{tikzcd}
\end{center}
%
i.e. $\phi(h(a))\boldsymbol{\pi}_{1}(a)=\boldsymbol{\pi}_{2}(a)\phi(t(a))$. We say that $\phi$ is an isomorphism if $\phi(x)$ is invertible for all $x$.
\end{definition}

%%%%%%%%%%End of DEFINITION %%%%%%%%%%%

For any two representations $\boldsymbol{\pi}_{1}$ and $\boldsymbol{\pi}_{2}$ of a quiver $Q$, their direct sum is given according to $(\boldsymbol{\pi}_{1}\oplus\boldsymbol{\pi}_{2})(x)=\boldsymbol{\pi}_{1}(x)\oplus\boldsymbol{\pi}_{2}(x)$ whether $x$ is in $Q_{0}$ or $Q_{1}$~\cite{derksen2017introduction}. Additionally, we will call a representation $\boldsymbol{\pi}$ trivial if $\boldsymbol{\pi}(x)=\mathbf{0}$ for all $x\in Q_{0}$.

Now, we are ready to introduce the notion of decomposable (indecomposable) and irreducible representation. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
A nontrivial representation $\boldsymbol{\pi}$ of a quiver $Q$ is called decomposable if $\boldsymbol{\pi}$ is isomorphic to $(\boldsymbol{\pi}_{1}\oplus\boldsymbol{\pi}_{2})$ for some nontrivial representations 
$\boldsymbol{\pi}_{1}, \boldsymbol{\pi}_{2}$ of $Q$. A nontrivial representation that is not decomposable is called indecomposable. A nontrivial representation $\boldsymbol{\pi}$ is called irreducible or simple if for every subrepresentation $\boldsymbol{\theta}$ of $\boldsymbol{\pi}$, $\boldsymbol{\theta}$ is trivial or equal to $\boldsymbol{\pi}$.
\end{definition}

%%%%%%%%%%End of DEFINITION %%%%%%%%%%%

It is important to point out that this notion of representation is connected indeed connected with the traditional notions of decomposability and irreducibility for associative algebras~\cite{derksen2017introduction,repthysmbook} considering the so called \textit{path algebra}. A path $p$ in a quiver $Q=(Q_{0},Q_{1},h,t)$ of length $\ell\geq 1$ is a sequence $q=a_{\ell}a_{\ell-1}\ldots a_{1}$ of arrows in $Q_{1}$ such that $t(a_{i+1})=h(a_{i})$ for $i=1,\ldots,\ell-1$ with $h(p)=h(a_{\ell})$ and $t(p)=t(a_{1})$~\cite{derksen2017introduction}. In this context a trivial path $e_{x}$ of length zero can be defined by $h(e_{x})=t(e_{x})=x$. If $\boldsymbol{\pi}$ is a representation of Q, we can the define $\boldsymbol{\pi}(p)=\boldsymbol{\pi}(a_{\ell})\boldsymbol{\pi}(a_{\ell-1})\cdots \boldsymbol{\pi}(a_{1})$ and for $x\in Q_{0}$ we can define $\boldsymbol{\pi}(e_{x}):=1_{\boldsymbol{\pi}(x)}:\boldsymbol{\pi}(x)\rightarrow\boldsymbol{\pi}(x)$. Notice that for any paths $p,q$ we have that $\boldsymbol{\pi}(p)\boldsymbol{\pi}(q)=\boldsymbol{\pi}(pq)$ whenever $t(p)=h(q)$~\cite{derksen2017introduction,repthysmbook}.

\blue{---AlejandroPM: I am working here, I will improve this portion later----
The path algebra $\mathcal{A_{P}}$ is the $\mathbb{C}-$algebra with basis given by all the paths in $Q$. If we take any two elements $\vec{p},\vec{q}$ in $\mathcal{A_{P}}$, i.e. two paths $p,q$ in $Q$ we can define a product in $\mathcal{A_{P}}$ given by
%
\begin{equation}
\vec{p}\vec{q}=\left\lbrace
\begin{matrix}
\overrightarrow{pq}  & \text{if} & t(p)=h(q)\\
\vec{0}    & \text{if} &  t(p)\neq h(q)
\end{matrix}
\right.
\end{equation}
%
notice that $pq$ indicates the concatenation of paths.-----}

Relying on the associative algebra $\mathcal{A_{P}}$ we can formally define a signal processing framework in the sense of~\cite{algSP0,algSP1,algSP2,algSP3}, introduce then the notions of Fourier decompositions and unleash a complete theory of signal processing. Before we proceed to do so, we take into account that as pointed out in~\cite{derksen2017introduction} (page 12, proposition 1.5.4), the category\footnote{Here and after we use the word \textit{category} in the context of category theory.} of representations of a quiver is equivalent to the category of representations of its path algebra, this means that in terms of determining representations and its properties we can work either with the quiver directly or with its path algebra. However, As dicussed in~\cite{repthysmbook} (page 20, remark 2.8.7) in general it is easier to work with the representations of the quiver directly without using the path algebra.

Then, we proceed to develop the notion of signal processing on quivers under the umbrella of algebraic signal processing as stated in~\cite{algSP0,algSP1,algSP2,algSP3}, but working directly with the quiver representation. As we will show, we can define the notions of Fourier decomposition and filtering.














==> v02/sec_spquiverep.tex <==
%!TEX root = quiverSP_v00.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Signal Processing on Quiver Representations}
\label{sec:spquiverep}

We start with introducing the notion of \textit{signal} on the representation of a quiver as follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% DEFINITION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def:quiversig}
Let $Q=(Q_{0},Q_{1},h,t)$ a quiver and $\boldsymbol{\pi}$ a representation of $Q$. Then a signal $\mathbf{x}$ on $\boldsymbol{\pi}$ is defined according to the map
%
\begin{equation}
\mathbf{x}: Q_{0}\rightarrow\boldsymbol{\pi}(Q_{0}).
\end{equation}
%
\end{definition}

%%%%%% END DEFINITION %%%%%%%%%%%%%%

For the sake of clarity, in what follows we denote by the triple $(Q,\boldsymbol{\pi},\bbx)$ a quiver signal on the quiver $Q$ taking its values on the representation $\boldsymbol{\pi}$.

To illustrate what a signal on a quiver looks like let us consider the following example. 


%%--------------------------------------------------------------------
%%----------------------Example----------------------------------
%%--------------------------------------------------------------------

\begin{example}
Let us recall the examples and 1 and 2, where we discuss the quiver $Q$ illustrated in Fig.~\ref{xx}. An example of a signal $\bbx$ on $Q$ taking values in the representation $\boldsymbol{\pi}$ illustrated in example 2 is given by 
%
%
\begin{equation*}
\bbx(1)=[1,1]^{T},\quad \bbx(2)=2\bbI_{2\times 2},\quad\bbx(3)=5\bbI_{5\times 5}
\end{equation*}
%
%
\begin{equation*}
\bbx(4)=[1,0,1]^{T},\quad \bbx(5)=8
\end{equation*}
%
%
\end{example}

%%------------------End of Example---------------------------

Then a signal defined on the representation of a quiver assigns quantities of different \textit{nature} and dimension to every node of the quiver.

